Few and Fewer: Learning Better from Few Examples Using Fewer Base Classes

When training data is scarce, it is common to make use of a feature extractor that has been pre-trained on a large base dataset, either by fine-tuning its parameters on the ``target'' dataset or by directly adopting its representation as features for a simple classifier. Fine-tuning is ineffective for few-shot learning, since the target dataset contains only a handful of examples. However, directly adopting the features without fine-tuning relies on the base and target distributions being similar enough that these features achieve separability and generalization. This paper investigates whether better features for the target dataset can be obtained by training on fewer base classes, seeking to identify a more useful base dataset for a given task.We consider cross-domain few-shot image classification in eight different domains from Meta-Dataset and entertain multiple real-world settings (domain-informed, task-informed and uninformed) where progressively less detail is known about the target task. To our knowledge, this is the first demonstration that fine-tuning on a subset of carefully selected base classes can significantly improve few-shot learning. Our contributions are simple and intuitive methods that can be implemented in any few-shot solution. We also give insights into the conditions in which these solutions are likely to provide a boost in accuracy. We release the code to reproduce all experiments from this paper on GitHub. https://github.com/RafLaf/Few-and-Fewer.git

==> tables/claim1.tex <==
%\begin{table*}[!htbp]
%\caption{Few-Shot Accuracy on MD test split before/after finetuning on a subset on 10k FS tasks. The subsets were selected the target domain validation split}
%\begin{tabular}{c c c c c c c}
%\toprule
%& \multicolumn{2}{c}{MD} & \multicolumn{2}{c}{1 shot 5 ways} & \multicolumn{2}{c}{5 shot 5 ways} \\
%\hline
 %& Baseline & $\Delta$ DI Finetune & %Baseline & $\Delta$ DI Finetune & Baseline %& $\Delta$ DI Finetune \\
%\midrule
%Aircraft & 65.90 (± 0.23) & -3.69 (± 0.33) & 40.19 (± 0.17) & -0.81 (± 0.25) & 62.74 (± 0.19) & -2.82 (± 0.27) \\
%\hline
%CUB & 79.61 (± 0.22) & \textbf{+1.65 (± 0.30)} & 64.83 (± 0.23) & \textbf{+7.1 (± 0.32)} & 87.85 (± 0.14) & \textbf{+2.14 (± 0.18)} \\ \hline
%DTD & 75.85 (± 0.17) & \textbf{+1.17 (± 0.23)} & 44.87 (± 0.19) & \textbf{+4.48 (± 0.27)} & 69.97 (± 0.15) & \textbf{+2.79 (± 0.21)} \\ \hline
%Fungi & 51.73 (± 0.28) & \textbf{+0.15 (± 0.40)} & 52.36 (± 0.22) & \textbf{+1.47 (± 0.32)} & 75.28 (± 0.19) & \textbf{+0.48 (± 0.28)} \\ \hline
%Omniglot & 51.85 (± 0.31) & \textbf{+2.44 (± 0.45)} & 57.92 (± 0.26) & \textbf{+1.12 (± 0.37)} & 74.79 (± 0.21) & \textbf{+1.95 (± 0.30)} \\ \hline
%MSCOCO & 45.50 (± 0.24) & \textbf{+1.18 (± 0.34)} & 43.89 (± 0.20) & \textbf{+2.16 (± 0.29)} & 62.68 (± 0.19) & \textbf{+1.71 (± 0.27)} \\ \hline
%Traffic Signs & 53.86 (± 0.25) & -3.55 (± 0.35) & 57.83 (± 0.21) & -2.03 (± 0.29) & 73.78 (± 0.19) & -2.18 (± 0.28) \\ \hline
%VGG Flower & 92.32 (± 0.15) & -0.39 (± 0.2) & 75.27 (± 0.20) & \textbf{+1.52 (± 0.28)} & 94.20 (± 0.08) & -0.61 (± 0.12) \\ %\bottomrule
%\end{tabular}
%\label{claim1}
%\end{table*}



\begin{table*}[!htbp]
\caption{Few-Shot Accuracy on MD test split before/after finetuning on a subset on 10k FS tasks. The subsets were selected the target domain validation split}
\begin{tabular}{c c c c c c c}
\toprule
10k runs & \multicolumn{2}{c}{MD} & \multicolumn{2}{c}{5 shot 5 ways} & \multicolumn{2}{c}{1 shot 5 ways} \\
\midrule
 & Baseline & $\Delta$ DI Finetune & Baseline & $\Delta$ DI Finetune & Baseline & $\Delta$ DI Finetune \\
 \midrule
Aircraft & 65.90 (± 0.23) & -3.69 (± 0.33) & 62.74 (± 0.19) & -2.82 (± 0.27) & 40.19 (± 0.17) & -0.81 (± 0.25) \\

CUB & 79.61 (± 0.22) & \textbf{+1.65 (± 0.30)} & 87.85 (± 0.14) & \textbf{+2.14 (± 0.18)} & 64.83 (± 0.23) & \textbf{+7.10 (± 0.32)} \\
DTD & 75.85 (± 0.17) & \textbf{+1.17 (± 0.23)} & 69.97 (± 0.15) & \textbf{+2.79 (± 0.21)} & 44.87 (± 0.19) & \textbf{+4.48 (± 0.27)} \\
Fungi & 51.73 (± 0.28) & \textbf{+0.15 (± 0.4)} & 75.28 (± 0.19) & \textbf{+0.48 (± 0.28)} & 52.36 (± 0.22) & \textbf{+1.47 (± 0.32)} \\
Omniglot & 51.85 (± 0.31) & \textbf{+2.44 (± 0.45)} & 74.79 (± 0.21) & \textbf{+1.95 (± 0.30)} & 57.92 (± 0.26) & \textbf{+1.12 (± 0.37)} \\
MSCOCO & 45.50 (± 0.24) & \textbf{+1.18 (± 0.34)} & 62.68 (± 0.19) & \textbf{+1.71 (± 0.27)} & 43.89 (± 0.20) & \textbf{+2.16 (± 0.29)} \\
Traffic Signs & 53.86 (± 0.25) & -3.55 (± 0.35) & 73.78 (± 0.19) & -2.18 (± 0.28) & 57.83 (± 0.21) & -2.03 (± 0.29) \\
VGG Flower & 92.32 (± 0.15) & -0.39 (± 0.20) & 94.20 (± 0.08) & -0.61 (± 0.12) & 75.27 (± 0.20) & \textbf{+1.52 (± 0.28)} \\
\midrule
Average & 64.57 (± 0.16) & -0.13 (± 0.32) & 75.16 (± 0.08) &\textbf{+0.43 (± 0.17)} & 54.64 (± 0.13) & \textbf{+1.88 (± 0.26)} \\
\bottomrule
\end{tabular}
\end{table*}


==> tables/claim1_noDI.tex <==
\begin{tabular}{c  c c c c}
\toprule
10k runs  & \multicolumn{2}{c}{5 shot 5 ways} & \multicolumn{2}{c}{1 shot 5 ways} \\
\midrule
 & Baseline & $\Delta$ DI Finetune & Baseline & $\Delta$ DI Finetune \\
 \midrule
Aircraft &  62.74 (± 0.19) & -2.82 (± 0.27) & 40.19 (± 0.17) & -0.81 (± 0.25) \\

CUB  & 87.85 (± 0.14) & \textbf{+2.14 (± 0.18)} & 64.83 (± 0.23) & \textbf{+7.10 (± 0.32)} \\
DTD  & 69.97 (± 0.15) & \textbf{+2.79 (± 0.21)} & 44.87 (± 0.19) & \textbf{+4.48 (± 0.27)} \\
Fungi  & 75.28 (± 0.19) & \textbf{+0.48 (± 0.28)} & 52.36 (± 0.22) & \textbf{+1.47 (± 0.32)} \\
Omniglot  & 74.79 (± 0.21) & \textbf{+1.95 (± 0.30)} & 57.92 (± 0.26) & \textbf{+1.12 (± 0.37)} \\
MSCOCO  & 62.68 (± 0.19) & \textbf{+1.71 (± 0.27)} & 43.89 (± 0.20) & \textbf{+2.16 (± 0.29)} \\
Traffic Signs & 73.78 (± 0.19) & -2.18 (± 0.28) & 57.83 (± 0.21) & -2.03 (± 0.29) \\
VGG Flower  & 94.20 (± 0.08) & -0.61 (± 0.12) & 75.27 (± 0.20) & \textbf{+1.52 (± 0.28)} \\
\midrule
Average  & 75.16 (± 0.08) &\textbf{+0.43 (± 0.17)} & 54.64 (± 0.13) & \textbf{+1.88 (± 0.26)} \\
\bottomrule
\end{tabular}


==> tables/claim3DI.tex <==


\begin{table*}[!htbp]
\caption{Change of Few-Shot Accuracy on 10k FS tasks on MD test split after feature selection according to heuristics. Feature transforms were finetuned on clusters of classes. Different representations of source classes are used to cluster them: V: Visual, S: Semantic, R: Random and X: Concatenated Visual and Semantic. For each task a heuristic selects a feature transform. The heuristics are : SNR: Signal to Noise Ratio, LOO: Leave One Out accuracy, Sampling: Multivariate Normal sampling of validation points in latent space, Hard: Accuracy on support set, Soft: Confidence score on support set, RankMe: Described in~\cite{garrido2022rankme}, H&M: Prediction of accuracy with Homogeneity and Magnitude. We also added the Domain informed setting with Metadataset sampling}
\begin{adjustbox}{scale=0.8,center,margin=-0cm 0cm 0cm 0cm}
\begin{tabular}{cccccccccc}
\toprule
\toprule
&&$\Delta$ SNR & $\Delta$ LOO & $\Delta$ Sampling & $\Delta$  SSA & $\Delta$ SSC & $\Delta$ RankMe & $\Delta$ H\&M & DI\\
\midrule
\multirow{4}{*}{Aircraft}&V & +0.300 ±0.065 & -0.159 ±0.067 & +0.216 ±0.067 & +0.284 ±0.067 & -0.160 ±0.066 & +0.133 ±0.070 & +0.807 ±0.063 &\multirow{4}{*}{-3.69 (± 0.33)} \\
&S & -0.482 ±0.060 & -0.565 ±0.064 & -0.294 ±0.064 & -0.250 ±0.065 & -0.702 ±0.063 & +0.165 ±0.065 & -1.601 ±0.063 \\
&R & -3.840 ±0.069 & -0.420 ±0.057 & -0.071 ±0.056 & -0.106 ±0.056 & -2.218 ±0.072 & -0.907 ±0.056 & -0.725 ±0.055 \\
&X & +0.365 ±0.067 & -0.043 ±0.068 & +0.445 ±0.068 & +0.601 ±0.068 & +0.004 ±0.067 & +0.280 ±0.069 & \textbf{+1.133 ±0.064} \\
\midrule
\multirow{4}{*}{CUB}&V &  +0.671 ±0.040 & +1.053 ±0.046 & +1.469 ±0.047 & +1.295 ±0.047 & +0.910 ±0.047 & +1.910 ±0.047 & +0.408 ±0.044 &\multirow{4}{*}{+1.65 (± 0.30)} \\
&S & +0.989 ±0.041 & +1.280 ±0.045 & +1.681 ±0.047 & +1.569 ±0.047 & +1.264 ±0.046 & +2.052 ±0.047 & -0.066 ±0.043 \\
&R & -0.877 ±0.048 & +1.278 ±0.040 & +1.347 ±0.039 & +1.263 ±0.039 & +1.127 ±0.042 & +1.199 ±0.038 & +0.849 ±0.042 \\
&X & +0.752 ±0.040 & +1.141 ±0.046 & +1.524 ±0.047 & +1.372 ±0.047 & +1.048 ±0.047 & \textbf{+2.075 ±0.048} & +0.651 ±0.044 \\
\midrule
\multirow{4}{*}{DTD}&V & +1.412 ±0.073 & +1.838 ±0.079 & \textbf{+2.952 ±0.082} & +2.855 ±0.081 & +2.447 ±0.080 & +0.693 ±0.071 & +0.891 ±0.076 &\multirow{4}{*}{+1.17 (± 0.23)}\\
& S& +1.223 ±0.071 & +1.846 ±0.077 & +2.627 ±0.078 & +2.717 ±0.078 & +2.469 ±0.078 & -0.142 ±0.076 & +1.042 ±0.071 \\
& R& +0.125 ±0.076 & +1.667 ±0.068 & +1.981 ±0.066 & +1.998 ±0.066 & +0.848 ±0.073 & +1.447 ±0.063 & +1.269 ±0.065 \\
&X & +1.632 ±0.073 & +1.781 ±0.078 & +2.834 ±0.080 & +2.677 ±0.079 & +2.353 ±0.078 & +0.587 ±0.070 & +0.962 ±0.076 \\
\midrule
\multirow{4}{*}{Fungi}&V &  +1.162 ±0.060 & +0.937 ±0.064 & +0.885 ±0.065 & +0.842 ±0.065 & +0.984 ±0.065 & +1.266 ±0.063 & -0.626 ±0.066 & \multirow{4}{*}{ +0.15 (± 0.4)}\\
&S & +1.162 ±0.061 & +1.115 ±0.061 & +1.018 ±0.064 & +1.102 ±0.062 & +1.076 ±0.063 & +0.859 ±0.065 & +1.251 ±0.060 \\
&R & \textbf{+1.484 ±0.068} & +1.391 ±0.059 & +1.295 ±0.057 & +1.311 ±0.057 & +1.292 ±0.062 & +1.257 ±0.057 & +1.251 ±0.057 \\
&X & +1.214 ±0.061 & +0.969 ±0.064 & +0.846 ±0.065 & +0.820 ±0.065 & +1.065 ±0.064 & +1.267 ±0.063 & -0.460 ±0.065 \\
\midrule
\multirow{4}{*}{Omniglot}&V &  -0.567 ±0.077 & +0.141 ±0.075 & \textbf{+0.836 ±0.074} & +0.439 ±0.075 & -0.449 ±0.075 & +0.277 ±0.077 & -0.843 ±0.073 & \multirow{4}{*}{+2.44 (± 0.45)}\\
&S & -0.234 ±0.157 & +0.224 ±0.158 & +0.734 ±0.157 & +0.296 ±0.156 & -0.507 ±0.156 & +0.113 ±0.154 & -2.217 ±0.156 \\
&R & +0.025 ±0.063 & +0.164 ±0.063 & +0.474 ±0.063 & +0.390 ±0.062 & -0.001 ±0.063 & +0.199 ±0.062 & +0.071 ±0.061 \\
&X & -0.789 ±0.156 & +0.030 ±0.156 & +0.774 ±0.155 & +0.343 ±0.156 & -0.474 ±0.156 & +0.296 ±0.156 & -0.940 ±0.154 \\
\midrule
\multirow{4}{*}{MSCOCO}&V &  +0.155 ±0.046 & +0.525 ±0.050 & +1.178 ±0.049 & +1.149 ±0.050 & +0.543 ±0.050 & -0.312 ±0.045 & -1.508 ±0.047 &\multirow{4}{*}{+1.18 (± 0.34)}\\
&S & +0.583 ±0.040 & +0.601 ±0.047 & \textbf{+1.310 ±0.047} & +1.184 ±0.048 & +0.656 ±0.046 & -0.566 ±0.046 & -1.963 ±0.050 \\
&R & +0.484 ±0.044 & +1.068 ±0.040 & +1.200 ±0.038 & +1.230 ±0.039 & +0.618 ±0.042 & +1.080 ±0.039 & +1.112 ±0.039 \\
&X & +0.099 ±0.046 & +0.442 ±0.049 & +0.934 ±0.049 & +0.890 ±0.049 & +0.340 ±0.049 & +0.007 ±0.044 & -1.591 ±0.047 \\
\midrule
\multirow{4}{*}{Traffic Signs}&V &  +0.272 ±0.048 & -0.016 ±0.047 & +0.598 ±0.044 & +0.412 ±0.045 & -1.054 ±0.048 & -3.356 ±0.045 & -0.990 ±0.043 & \multirow{4}{*}{-3.55 (± 0.35)}\\
&S & -0.374 ±0.108 & +0.046 ±0.109 & +0.513 ±0.108 & +0.396 ±0.108 & -0.576 ±0.110 & -0.402 ±0.108 & +0.394 ±0.107 \\
&R & -0.668 ±0.035 & -0.491 ±0.037 & -0.003 ±0.035 & -0.097 ±0.035 & -0.743 ±0.040 & -0.949 ±0.035 & +0.115 ±0.036 \\
&X & +0.962 ±0.110 & +0.421 ±0.110 & \textbf{+1.083 ±0.108} & +0.896 ±0.108 & -0.541 ±0.111 & -2.695 ±0.110 & -0.641 ±0.107 \\
\midrule
\multirow{4}{*}{VGG Flower}&V &  +0.245 ±0.039 & +0.444 ±0.039 & +0.465 ±0.039 & +0.542 ±0.039 & +0.630 ±0.039 & +0.250 ±0.041 & -0.629 ±0.040 &\multirow{4}{*}{-0.39 (± 0.20)}\\
&S & +0.436 ±0.039 & +0.559 ±0.039 & +0.691 ±0.039 & +0.657 ±0.039 & +0.729 ±0.038 & \textbf{+0.945 ±0.038} & -0.038 ±0.040 \\
&R & +0.188 ±0.044 & +0.420 ±0.036 & +0.567 ±0.034 & +0.497 ±0.034 & +0.526 ±0.037 & +0.826 ±0.034 & +0.456 ±0.034 \\
&X & +0.249 ±0.039 & +0.417 ±0.039 & +0.438 ±0.039 & +0.511 ±0.039 & +0.624 ±0.038 & +0.223 ±0.041 & -0.817 ±0.040 \\
\midrule
Average & & +0.751 ±0.029 & +0.734 ±0.029 & \textbf{+1.040 ±0.029} & +0.968 ±0.029 & +0.906 ±0.030 & +0.898 ±0.028 & +0.885 ±0.028 & -0.13 (± 0.32)\\
\bottomrule
\end{tabular}
\end{adjustbox}
\label{claim3_1}
\end{table*}



==> tables/claim3_1.tex <==


\begin{table*}[!htbp]
\caption{Change of Few-Shot Accuracy on 10k FS tasks on MD test split after feature selection according to heuristics. Feature transforms were finetuned on clusters of classes. Different representations of source classes are used to cluster them: V: Visual, S: Semantic, R: Random and X: Concatenated Visual and Semantic. For each task a heuristic selects a feature transform. The heuristics are : SNR: Signal to Noise Ratio, LOO: Leave One Out accuracy, Sampling: Multivariate Normal sampling of validation points in latent space, Hard: Accuracy on support set, Soft: Confidence score on support set, RankMe: Described in~\cite{garrido2022rankme}, H&M: Prediction of accuracy with Homogeneity and Magnitude }
\begin{adjustbox}{scale=0.9,center,margin=-0cm 0cm 0cm 0cm}
\begin{tabular}{ccccccccc}
\toprule
\toprule
&&$\Delta$ SNR & $\Delta$ LOO & $\Delta$ Sampling & $\Delta$  Hard & $\Delta$ Soft & $\Delta$ RankMe & $\Delta$ H\&M\\
\midrule
\multirow{4}{*}{Aircraft}&V & +0.300 ±0.065 & -0.159 ±0.067 & +0.216 ±0.067 & +0.284 ±0.067 & -0.160 ±0.066 & +0.133 ±0.070 & +0.807 ±0.063 \\
&S & -0.482 ±0.060 & -0.565 ±0.064 & -0.294 ±0.064 & -0.250 ±0.065 & -0.702 ±0.063 & +0.165 ±0.065 & -1.601 ±0.063 \\
&R & -3.840 ±0.069 & -0.420 ±0.057 & -0.071 ±0.056 & -0.106 ±0.056 & -2.218 ±0.072 & -0.907 ±0.056 & -0.725 ±0.055 \\
&X & +0.365 ±0.067 & -0.043 ±0.068 & +0.445 ±0.068 & +0.601 ±0.068 & +0.004 ±0.067 & +0.280 ±0.069 & \textbf{+1.133 ±0.064} \\
\midrule
\multirow{4}{*}{CUB}&V &  +0.671 ±0.040 & +1.053 ±0.046 & +1.469 ±0.047 & +1.295 ±0.047 & +0.910 ±0.047 & +1.910 ±0.047 & +0.408 ±0.044 \\
&S & +0.989 ±0.041 & +1.280 ±0.045 & +1.681 ±0.047 & +1.569 ±0.047 & +1.264 ±0.046 & +2.052 ±0.047 & -0.066 ±0.043 \\
&R & -0.877 ±0.048 & +1.278 ±0.040 & +1.347 ±0.039 & +1.263 ±0.039 & +1.127 ±0.042 & +1.199 ±0.038 & +0.849 ±0.042 \\
&X & +0.752 ±0.040 & +1.141 ±0.046 & +1.524 ±0.047 & +1.372 ±0.047 & +1.048 ±0.047 & \textbf{+2.075 ±0.048} & +0.651 ±0.044 \\
\midrule
\multirow{4}{*}{DTD}&V & +1.412 ±0.073 & +1.838 ±0.079 & \textbf{+2.952 ±0.082} & +2.855 ±0.081 & +2.447 ±0.080 & +0.693 ±0.071 & +0.891 ±0.076 \\
& S& +1.223 ±0.071 & +1.846 ±0.077 & +2.627 ±0.078 & +2.717 ±0.078 & +2.469 ±0.078 & -0.142 ±0.076 & +1.042 ±0.071 \\
& R& +0.125 ±0.076 & +1.667 ±0.068 & +1.981 ±0.066 & +1.998 ±0.066 & +0.848 ±0.073 & +1.447 ±0.063 & +1.269 ±0.065 \\
&X & +1.632 ±0.073 & +1.781 ±0.078 & +2.834 ±0.080 & +2.677 ±0.079 & +2.353 ±0.078 & +0.587 ±0.070 & +0.962 ±0.076 \\
\midrule
\multirow{4}{*}{Fungi}&V &  +1.162 ±0.060 & +0.937 ±0.064 & +0.885 ±0.065 & +0.842 ±0.065 & +0.984 ±0.065 & +1.266 ±0.063 & -0.626 ±0.066 \\
&S & +1.162 ±0.061 & +1.115 ±0.061 & +1.018 ±0.064 & +1.102 ±0.062 & +1.076 ±0.063 & +0.859 ±0.065 & +1.251 ±0.060 \\
&R & \textbf{+1.484 ±0.068} & +1.391 ±0.059 & +1.295 ±0.057 & +1.311 ±0.057 & +1.292 ±0.062 & +1.257 ±0.057 & +1.251 ±0.057 \\
&X & +1.214 ±0.061 & +0.969 ±0.064 & +0.846 ±0.065 & +0.820 ±0.065 & +1.065 ±0.064 & +1.267 ±0.063 & -0.460 ±0.065 \\
\midrule
\multirow{4}{*}{Omniglot}&V &  -0.567 ±0.077 & +0.141 ±0.075 & \textbf{+0.836 ±0.074} & +0.439 ±0.075 & -0.449 ±0.075 & +0.277 ±0.077 & -0.843 ±0.073 \\
&S & -0.234 ±0.157 & +0.224 ±0.158 & +0.734 ±0.157 & +0.296 ±0.156 & -0.507 ±0.156 & +0.113 ±0.154 & -2.217 ±0.156 \\
&R & +0.025 ±0.063 & +0.164 ±0.063 & +0.474 ±0.063 & +0.390 ±0.062 & -0.001 ±0.063 & +0.199 ±0.062 & +0.071 ±0.061 \\
&X & -0.789 ±0.156 & +0.030 ±0.156 & +0.774 ±0.155 & +0.343 ±0.156 & -0.474 ±0.156 & +0.296 ±0.156 & -0.940 ±0.154 \\
\midrule
\multirow{4}{*}{MSCOCO}&V &  +0.155 ±0.046 & +0.525 ±0.050 & +1.178 ±0.049 & +1.149 ±0.050 & +0.543 ±0.050 & -0.312 ±0.045 & -1.508 ±0.047 \\
&S & +0.583 ±0.040 & +0.601 ±0.047 & \textbf{+1.310 ±0.047} & +1.184 ±0.048 & +0.656 ±0.046 & -0.566 ±0.046 & -1.963 ±0.050 \\
&R & +0.484 ±0.044 & +1.068 ±0.040 & +1.200 ±0.038 & +1.230 ±0.039 & +0.618 ±0.042 & +1.080 ±0.039 & +1.112 ±0.039 \\
&X & +0.099 ±0.046 & +0.442 ±0.049 & +0.934 ±0.049 & +0.890 ±0.049 & +0.340 ±0.049 & +0.007 ±0.044 & -1.591 ±0.047 \\
\midrule
\multirow{4}{*}{Traffic Signs}&V &  +0.272 ±0.048 & -0.016 ±0.047 & +0.598 ±0.044 & +0.412 ±0.045 & -1.054 ±0.048 & -3.356 ±0.045 & -0.990 ±0.043 \\
&S & -0.374 ±0.108 & +0.046 ±0.109 & +0.513 ±0.108 & +0.396 ±0.108 & -0.576 ±0.110 & -0.402 ±0.108 & +0.394 ±0.107 \\
&R & -0.668 ±0.035 & -0.491 ±0.037 & -0.003 ±0.035 & -0.097 ±0.035 & -0.743 ±0.040 & -0.949 ±0.035 & +0.115 ±0.036 \\
&X & +0.962 ±0.110 & +0.421 ±0.110 & \textbf{+1.083 ±0.108} & +0.896 ±0.108 & -0.541 ±0.111 & -2.695 ±0.110 & -0.641 ±0.107 \\
\midrule
\multirow{4}{*}{VGG Flower}&V &  +0.245 ±0.039 & +0.444 ±0.039 & +0.465 ±0.039 & +0.542 ±0.039 & +0.630 ±0.039 & +0.250 ±0.041 & -0.629 ±0.040 \\
&S & +0.436 ±0.039 & +0.559 ±0.039 & +0.691 ±0.039 & +0.657 ±0.039 & +0.729 ±0.038 & \textbf{+0.945 ±0.038} & -0.038 ±0.040 \\
&R & +0.188 ±0.044 & +0.420 ±0.036 & +0.567 ±0.034 & +0.497 ±0.034 & +0.526 ±0.037 & +0.826 ±0.034 & +0.456 ±0.034 \\
&X & +0.249 ±0.039 & +0.417 ±0.039 & +0.438 ±0.039 & +0.511 ±0.039 & +0.624 ±0.038 & +0.223 ±0.041 & -0.817 ±0.040 \\
\midrule

Average & & +0.751 ±0.029 & +0.734 ±0.029 & \textbf{+1.040 ±0.029} & +0.968 ±0.029 & +0.906 ±0.030 & +0.898 ±0.028 & +0.885 ±0.028 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\label{claim3_1}
\end{table*}


%\begin{table*}[!htbp]
%\caption{Few-Shot Accuracy on MD test split before/after finetuning on a subset on 10k FS tasks. The subsets were selected the target domain validation split}
%\begin{tabular}{cccccccc}
%\toprule
%&& $\Delta$ SNR & $\Delta$ LOO & $\Delta$ Sampling & $\Delta$  Hard & $\Delta$ Soft & $\Delta$ RankMe \\
%\midrule
%\multirow{3}{*}{Aircraft}& V & +0.300 ±0.065 & -0.148 ±0.068 & +0.213 ±0.067 & +0.220 ±0.068 & -0.157 ±0.066 & +0.133 ±0.070 \\
%&S & -1.107 ±0.060 & -0.674 ±0.065 & -0.194 ±0.066 & -0.048 ±0.067 & -1.101 ±0.062 & \textbf{+0.363 ±0.066} \\
%&R & -3.838 ±0.069 & -0.510 ±0.057 & -0.082 ±0.056 & -0.179 ±0.057 & -2.217 ±0.072 & -0.903 ±0.056 \\
%\midrule
%\multirow{3}{*}{CUB} &V & +0.671 ±0.040 & +1.128 ±0.045 & +1.532 ±0.047 & +1.467 ±0.046 & +0.918 ±0.047 & +1.910 ±0.047 \\
%&S & +0.683 ±0.041 & +1.207 ±0.044 & +1.587 ±0.046 & +1.470 ±0.045 & +1.078 ±0.046 & \textbf{+1.926 ±0.047} \\
%&R & -0.877 ±0.048 & +1.329 ±0.040 & +1.403 ±0.039 & +1.422 ±0.040 & +1.157 ±0.042 & +1.222 ±0.038 \\
%\midrule
%\multirow{3}{*}{DTD} &V & +1.412 ±0.073 & +1.778 ±0.079 & +2.908 ±0.082 & +2.766 ±0.082 & +2.415 ±0.080 & +0.696 ±0.071 \\
%&S & +1.229 ±0.071 & +1.964 ±0.077 & +2.800 ±0.079 & \textbf{+2.973 ±0.080} & +2.558 ±0.078 & +0.121 ±0.075 \\
%&R & +0.125 ±0.076 & +1.588 ±0.069 & +1.964 ±0.066 & +1.939 ±0.067 & +0.821 ±0.074 & +1.450 ±0.063 \\
%\midrule
%\multirow{3}{*}{Fungi} &V & +1.162 ±0.060 & +0.912 ±0.065 & +0.877 ±0.065 & +0.860 ±0.066 & +0.996 ±0.065 & +1.214 ±0.063 \\
%&S & +1.274 ±0.062 & +1.150 ±0.062 & +0.937 ±0.065 & +0.910 ±0.065 & +1.047 ±0.064 & +0.946 ±0.064 \\
%&R & \textbf{+1.484 ±0.068} & +1.389 ±0.060 & +1.287 ±0.057 & +1.301 ±0.057 & +1.285 ±0.061 & +1.299 ±0.057\\
%\midrule
%\multirow{3}{*}{Omniglot} &V & -0.567 ±0.077 & -0.077 ±0.077 & +0.640 ±0.077 & -0.037 ±0.080 & -0.739 ±0.077 & +0.277 ±0.077 \\
%&S & -0.340 ±0.074 & +0.150 ±0.075 & \textbf{+0.665 ±0.074} & +0.213 ±0.075 & -0.599 ±0.073 & +0.258 ±0.069 \\
%&R & -0.036 ±0.063 & +0.022 ±0.064 & +0.350 ±0.063 & +0.027 ±0.064 & -0.154 ±0.064 & +0.190 ±0.062 \\
%\midrule
%\multirow{3}{*}{MSCOCO} &V & +0.155 ±0.046 & +0.553 ±0.050 & +1.180 ±0.049 & +1.183 ±0.049 & +0.555 ±0.050 & -0.330 ±0.045 \\
%&S & +0.560 ±0.041 & +0.756 ±0.047 & \textbf{+1.281 ±0.047} & +1.173 ±0.048 & +0.694 ±0.045 & +0.205 ±0.046 \\
%&R & +0.484 ±0.044 & +1.043 ±0.040 & +1.202 ±0.038 & +1.196 ±0.039 & +0.608 ±0.042 & +1.096 ±0.040 \\
%\midrule
%\multirow{3}{*}{Traffic Signs} &V & +0.272 ±0.048 & +0.027 ±0.047 & %\textbf{+0.612 ±0.044} & +0.441 ±0.045 & -1.060 ±0.048 & -3.356 ±0.045 \\
%&S & +0.080 ±0.043 & -0.007 ±0.045 & +0.475 ±0.043 & +0.370 ±0.043 & -0.721 ±0.050 & -0.659 ±0.041 \\
%&R & -0.667 ±0.035 & -0.449 ±0.036 & +0.009 ±0.035 & -0.070 ±0.035 & -0.719 ±0.039 & -0.917 ±0.036 \\
%\midrule
%\multirow{3}{*}{VGG Flower} &V & +0.245 ±0.039 & +0.389 ±0.039 & +0.440 ±0.039 & +0.345 ±0.039 & +0.581 ±0.039 & +0.250 ±0.041 \\
%&S  & +0.330 ±0.038 & +0.466 ±0.038 & +0.638 ±0.038 & +0.493 ±0.038 & +0.632 ±0.038 & \textbf{+0.884 ±0.038 }\\
%&R  & +0.188 ±0.044 & +0.444 ±0.036 & +0.589 ±0.034 & +0.534 ±0.034 & +0.531 ±0.037 & +0.826 ±0.034 \\
%\bottomrule
%\end{tabular}
%\end{table*}

==> tables/others_not_included.tex <==
\begin{table}
\center
\begin{tabular}{c|c|c|c|c|c|c|}
\cline{2-7}
 & \multicolumn{6}{c|}{Dataset} \\
\cline{2-7}
 &\multicolumn{3}{c|}{Aircraft} & \multicolumn{3}{c|}{CUB} \\
\cline{2-7}
&TA & TA+DI & TA+TI & TA & TA+DI & TA+TI\\
\hline
\multicolumn{1}{|c|}{SNR} & x& x& x& x& x& x\\
\hline
\multicolumn{1}{|c|}{LOO}& x& x& x& x& x& x\\
\hline\multicolumn{1}{|c|}{Oracle} & x& x& x& x& x& x\\
\hline
\end{tabular}
\caption{1-shot 5 ways}
\end{table}


\begin{table}
\begin{center}
\begin{tabular}{ |c|c|c|c| } 
\hline
\makecell{Info. \\ Available} & Method &\makecell{ Domain \\ required} & \makecell{Labels\\ required }\\
\hline
\multirow{2}{4em}{\centering Domain informed} & Activation & \checkmark & \\ 
\cline{2-4}
& 1DA & \checkmark & \checkmark\\ 
\hline{}
\multirow{2}{4em}{\centering FS task informed} & Activation & \ & \\ 
\cline{2-4}
& 1DA &  & \checkmark\\ 
\hline
\multirow{3}{4em}{\centering Problem Agnostic} & VHC & & \\ 
\cline{2-4}
& SHC & & \\ 
\cline{2-4}
& Random & &  \\ 
\hline
\end{tabular}
\end{center}
\caption{Methods depending on the information available. VHC and SHC stand for respectively Visual Hierarchical Clustering and Semantic Hierarchical Clustering}
\label{table_info}
\end{table}

==> tables/out_table.tex <==
\begin{tabular}{cccccccc}
\multirow{2}{*}{Dataset} & \multirow{2}{*}{Method} & \multicolumn{2}{c}{1-shot 5-ways} & \multicolumn{2}{c}{5-shots 5-ways} & \multicolumn{2}{c}{MD} \\
                      \cmidrule(lr){3-8} 
                      &        &     Baseline &      $\Delta$ &     Baseline &      $\Delta$ &     Baseline &      $\Delta$ \\
\midrule
     \multirow{3}{*}{Aircraft} &      S & \multirow{3}{*}{39.947 ±0.697} &          -3.602 ±0.635 & \multirow{3}{*}{63.176 ±0.738} &          -1.480 ±0.615 & \multirow{3}{*}{65.865 ±0.904} & \textbf{+5.335 ±0.692} \\
                               &     TI &                                &          -0.064 ±0.326 &                                &          +0.264 ±0.309 &                                &          +1.328 ±0.250 \\
                               &     DI &                                & \textbf{+0.342 ±0.323} &                                & \textbf{+0.540 ±0.308} &                                &          +1.320 ±0.269 \\
                               \midrule
          \multirow{3}{*}{CUB} &      S & \multirow{3}{*}{64.340 ±0.895} &         -19.278 ±0.877 & \multirow{3}{*}{87.780 ±0.587} &         -18.971 ±0.633 & \multirow{3}{*}{79.289 ±0.904} &         -14.506 ±0.598 \\
                               &     TI &                                &          +2.642 ±0.442 &                                &          +2.160 ±0.261 &                                &          +1.083 ±0.187 \\
                               &     DI &                                & \textbf{+3.269 ±0.441} &                                & \textbf{+2.291 ±0.260} &                                & \textbf{+2.202 ±0.200} \\\midrule
          \multirow{3}{*}{DTD} &      S & \multirow{3}{*}{45.211 ±0.770} &          +0.656 ±0.772 & \multirow{3}{*}{70.096 ±0.595} &          -3.116 ±0.590 & \multirow{3}{*}{76.025 ±0.693} &          -6.665 ±0.685 \\
                               &     TI &                                &          +2.849 ±0.462 &                                &          +2.773 ±0.327 &                                &          +2.443 ±0.293 \\
                               &     DI &                                & \textbf{+2.896 ±0.478} &                                & \textbf{+2.958 ±0.328} &                                & \textbf{+2.784 ±0.310} \\\midrule
        \multirow{3}{*}{Fungi} &      S & \multirow{3}{*}{53.006 ±0.918} &          -6.594 ±0.743 & \multirow{3}{*}{74.868 ±0.795} &          -8.329 ±0.616 & \multirow{3}{*}{51.570 ±1.160} &         -15.054 ±0.534 \\
                               &     TI &                                &          +0.915 ±0.390 &                                &          +1.665 ±0.300 &                                &          +1.068 ±0.256 \\
                               &     DI &                                & \textbf{+1.071 ±0.412} &                                & \textbf{+1.891 ±0.291} &                                & \textbf{+1.378 ±0.252} \\\midrule
     \multirow{3}{*}{Omniglot} &      S & \multirow{3}{*}{61.796 ±1.033} &          -3.160 ±1.110 & \multirow{3}{*}{81.533 ±0.761} &          +3.529 ±0.852 & \multirow{3}{*}{59.512 ±1.309} &          -4.592 ±1.067 \\
                               &     TI &                                &          +2.647 ±0.382 &                                &          +2.936 ±0.290 &                                &          +3.744 ±0.235 \\
                               &     DI &                                & \textbf{+3.522 ±1.222} &                                & \textbf{+3.573 ±0.810} &                                & \textbf{+3.926 ±0.614} \\\midrule
       \multirow{3}{*}{MSCOCO} &      S & \multirow{3}{*}{43.911 ±0.848} &          -5.442 ±0.658 & \multirow{3}{*}{63.044 ±0.786} &          -6.200 ±0.632 & \multirow{3}{*}{44.986 ±0.988} &         -16.999 ±0.717 \\
                               &     TI &                                &          +1.273 ±0.349 &                                &          +1.869 ±0.286 &                                &          +1.852 ±0.166 \\
                               &     DI &                                & \textbf{+1.616 ±0.342} &                                & \textbf{+2.089 ±0.296} &                                & \textbf{+2.252 ±0.166} \\\midrule
\multirow{3}{*}{Traffic Signs} &      S & \multirow{3}{*}{57.347 ±0.852} &          -4.667 ±0.661 & \multirow{3}{*}{74.113 ±0.781} & \textbf{+6.173 ±0.622} & \multirow{3}{*}{53.769 ±1.051} & \textbf{+0.765 ±0.997} \\
                               &     TI &                                &          -0.844 ±0.323 &                                &          -1.224 ±0.254 &                                &          -2.018 ±0.175 \\
                               &     DI &                                & \textbf{-0.787 ±0.947} &                                &          -1.476 ±0.769 &                                &          -1.824 ±0.436 \\\midrule
   \multirow{3}{*}{VGG Flower} &      S & \multirow{3}{*}{75.864 ±0.845} &          +0.187 ±0.792 & \multirow{3}{*}{94.456 ±0.326} &          -1.453 ±0.366 & \multirow{3}{*}{92.769 ±0.579} &          -5.183 ±0.507 \\
                               &     TI &                                & \textbf{+2.038 ±0.398} &                                & \textbf{+0.636 ±0.177} &                                & \textbf{+1.030 ±0.158} \\
                               &     DI &                                &          +1.880 ±0.406 &                                &          +0.520 ±0.176 &                                &          +0.836 ±0.158 \\
\bottomrule
\end{tabular}




==> tables/out_uot.tex <==
\begin{tabular}{cccccccc}
\multirow{2}{*}{Dataset} & \multirow{2}{*}{Method} & \multicolumn{2}{c}{1-shot 5-ways} & \multicolumn{2}{c}{5-shots 5-ways} & \multicolumn{2}{c}{MD} \\
                      \cmidrule(lr){3-8} 
                      &        &     Baseline &      $\Delta$ &     Baseline &      $\Delta$ &     Baseline &      $\Delta$ \\
\midrule
\midrule
     \multirow{4}{*}{Aircraft} &      S & \multirow{4}{*}{39.95 ±0.70} &          -3.60 ±0.64 & \multirow{4}{*}{63.18 ±0.74} &          -1.48 ±0.61 & \multirow{4}{*}{65.86 ±0.90} & \textbf{+5.33 ±0.69} \\
                               &     TI &                              &          -0.06 ±0.33 &                              &          \textbf{+0.26 ±0.31} &                              &          +1.33 ±0.25 \\
                               &     DI &                              & \textbf{+0.34 ±0.32} &                              & \textbf{+0.54 ±0.31} &                              &          +1.32 ±0.27 \\
                               & DI-UOT &                              &          -0.25 ±0.33 &                              &          -0.04 ±0.30 &                              &          +0.86 ±0.27 \\ \midrule
          \multirow{4}{*}{CUB} &      S & \multirow{4}{*}{64.34 ±0.90} &         -19.28 ±0.88 & \multirow{4}{*}{87.78 ±0.59} &         -18.97 ±0.63 & \multirow{4}{*}{79.29 ±0.90} &         -14.51 ±0.60 \\
                               &     TI &                              &          +2.64 ±0.44 &                              &          \textbf{+2.16 ±0.26} &                              &          +1.08 ±0.19 \\
                               &     DI &                              & \textbf{+3.27 ±0.44} &                              & \textbf{+2.29 ±0.26} &                              & \textbf{+2.20 ±0.20} \\
                               & DI-UOT &                              &          +2.99 ±0.43 &                              &          \textbf{+2.07 ±0.27} &                              &          \textbf{+1.97 ±0.20} \\ \midrule
          \multirow{4}{*}{DTD} &      S & \multirow{4}{*}{45.21 ±0.77} &          +0.66 ±0.77 & \multirow{4}{*}{70.10 ±0.59} &          -3.12 ±0.59 & \multirow{4}{*}{76.03 ±0.69} &          -6.67 ±0.69 \\
                               &     TI &                              &          \textbf{+2.85 ±0.46} &                              &          \textbf{+2.77 ±0.33} &                              &          \textbf{+2.44 ±0.29} \\
                               &     DI &                              & \textbf{+2.90 ±0.48} &                              & \textbf{+2.96 ±0.33} &                              &          \textbf{+2.78 ±0.31} \\
                               & DI-UOT &                              &          \textbf{+2.26 ±0.51} &                              &          \textbf{+2.62 ±0.34} &                              & \textbf{+2.82 ±0.32} \\ \midrule
        \multirow{4}{*}{Fungi} &      S & \multirow{4}{*}{53.01 ±0.92} &          -6.59 ±0.74 & \multirow{4}{*}{74.87 ±0.80} &          -8.33 ±0.62 & \multirow{4}{*}{51.57 ±1.16} &         -15.05 ±0.53 \\
                               &     TI &                              &          \textbf{+0.92 ±0.39} &                              &         \textbf{+1.67 ±0.30} &                              &          \textbf{+1.07 ±0.26} \\
                               &     DI &                              & \textbf{+1.07 ±0.41} &                              & \textbf{+1.89 ±0.29} &                              & \textbf{+1.38 ±0.25} \\
                               & DI-UOT &                              &          +0.74 ±0.40 &                              &          \textbf{+1.46 ±0.29} &                              &         \textbf{ +0.91 ±0.25} \\ \midrule
     \multirow{4}{*}{Omniglot} &      S & \multirow{4}{*}{61.80 ±1.03} &          -3.16 ±1.11 & \multirow{4}{*}{81.53 ±0.76} &          \textbf{+3.53 ±0.85} & \multirow{4}{*}{59.51 ±1.31} &          -4.59 ±1.07 \\
                               &     TI &                              &          \textbf{+2.65 ±0.38} &                              &          \textbf{+2.94 ±0.29} &                              &          \textbf{+3.74 ±0.23} \\
                               &     DI &                              & \textbf{+3.52 ±1.22} &                              & \textbf{+3.57 ±0.81} &                              & \textbf{+3.93 ±0.61} \\
                               & DI-UOT &                              &          -3.70 ±1.00 &                              &          -5.02 ±0.68 &                              &          -5.76 ±0.66 \\ \midrule
       \multirow{4}{*}{MSCOCO} &      S & \multirow{4}{*}{43.91 ±0.85} &          -5.44 ±0.66 & \multirow{4}{*}{63.04 ±0.79} &          -6.20 ±0.63 & \multirow{4}{*}{44.99 ±0.99} &         -17.00 ±0.72 \\
                               &     TI &                              &          \textbf{+1.27 ±0.35} &                              &          \textbf{+1.87 ±0.29} &                              &          +1.85 ±0.17 \\
                               &     DI &                              & \textbf{+1.62 ±0.34} &                              & \textbf{+2.09 ±0.30} &                              & \textbf{+2.25 ±0.17} \\
                               & DI-UOT &                              &          \textbf{+1.27 ±0.35} &                              &          \textbf{+1.75 ±0.29} &                              &          \textbf{+2.09 ±0.18} \\ \midrule
\multirow{4}{*}{Traffic Signs} &      S & \multirow{4}{*}{\textbf{57.35 ±0.85}} &          -4.67 ±0.66 & \multirow{4}{*}{74.11 ±0.78} & \textbf{+6.17 ±0.62} & \multirow{4}{*}{\textbf{53.77 ±1.05}} & \textbf{+0.77 ±1.00} \\
                               &     TI &                              &          \textbf{-0.84 ±0.32} &                              &          -1.22 ±0.25 &                              &          -2.02 ±0.17 \\
                               &     DI &                              &          \textbf{-0.79 ±0.95} &                              &          -1.48 ±0.77 &                              &          -1.82 ±0.44 \\
                               & DI-UOT &                              & \textbf{-0.48 ±0.33} &                              &          -0.64 ±0.27 &                              &          -1.26 ±0.18 \\ \midrule
   \multirow{4}{*}{VGG Flower} &      S & \multirow{4}{*}{75.86 ±0.84} &          +0.19 ±0.79 & \multirow{4}{*}{94.46 ±0.33} &          -1.45 ±0.37 & \multirow{4}{*}{92.77 ±0.58} &          -5.18 ±0.51 \\
                               &     TI &                              &          \textbf{+2.04 ±0.40} &                              &         \textbf{ +0.64 ±0.18} &                              & \textbf{+1.03 ±0.16} \\
                               &     DI &                              &          \textbf{+1.88 ±0.41} &                              &          \textbf{+0.52 ±0.18} &                              &          \textbf{+0.84 ±0.16} \\
                               & DI-UOT &                              & \textbf{+2.18 ±0.40} &                              & \textbf{+0.67 ±0.18} &                              &          \textbf{+0.90 ±0.16} \\ \midrule
      \multirow{4}{*}{Average} &      S &            \multirow{4}{*}{} &          -5.24 ±0.78 &            \multirow{4}{*}{} &          -3.73 ±0.61 &            \multirow{4}{*}{} &          -7.11 ±0.73 \\
                               &     TI &                              &          \textbf{+1.43 ±0.38} &                              &          \textbf{+1.39 ±0.28} &                              &          \textbf{+1.31 ±0.21} \\
                               &     DI &                              & \textbf{+1.73 ±0.57} &                              & \textbf{+1.55 ±0.41} &                              & \textbf{+1.61 ±0.30} \\
                               & DI-UOT &                              &          +0.63 ±0.47 &                              &          +0.36 ±0.33 &                              &          +0.32 ±0.28 \\
\bottomrule
\end{tabular}



==> tables/out_uot_updated.tex <==
\begin{tabular}{cccccccc}
\multirow{2}{*}{Dataset} & \multirow{2}{*}{Method} & \multicolumn{2}{c}{1-shot 5-ways} & \multicolumn{2}{c}{5-shots 5-ways} & \multicolumn{2}{c}{MD} \\
                      \cmidrule(lr){3-8} 
                      &        &     Baseline &      $\Delta$ &     Baseline &      $\Delta$ &     Baseline &      $\Delta$ \\
\midrule
\midrule
     \multirow{5}{*}{Aircraft} &      S & \multirow{5}{*}{39.95 ±0.70} &          -3.60 ±0.64 & \multirow{5}{*}{63.18 ±0.74} &          -1.48 ±0.61 & \multirow{5}{*}{65.86 ±0.90} & \textbf{+5.33 ±0.69} \\
                               &     TI &                              &          -0.06 ±0.33 &                              &          \textbf{+0.26 ±0.31} &                              &          +1.33 ±0.25 \\
                               &     DI &                              & \textbf{+0.34 ±0.32} &                              & \textbf{+0.54 ±0.31} &                              &          +1.32 ±0.27 \\
                               & DI-UOT &                              &          -0.25 ±0.33 &                              &          -0.04 ±0.30 &                              &          +0.86 ±0.27 \\
                               
                               & TI-UOT & &	-0.06 ±0.33 & &-0.01 ±0.30 & &+0.93 ±0.26 \\ \midrule
          \multirow{5}{*}{CUB} &      S & \multirow{5}{*}{64.34 ±0.90} &         -19.28 ±0.88 & \multirow{5}{*}{87.78 ±0.59} &         -18.97 ±0.63 & \multirow{5}{*}{79.29 ±0.90} &         -14.51 ±0.60 \\
                               &     TI &                              &          +2.64 ±0.44 &                              &          \textbf{+2.16 ±0.26} &                              &          +1.08 ±0.19 \\
                               &     DI &                              & \textbf{+3.27 ±0.44} &                              & \textbf{+2.29 ±0.26} &                              & \textbf{+2.20 ±0.20} \\
                               & DI-UOT &                              &          +2.99 ±0.43 &                              &          \textbf{+2.07 ±0.27} &                              &          \textbf{+1.97 ±0.20} \\
                               
                               & TI-UOT & & +2.64 ±0.44& &+1.11 ±0.26 & &+0.96 ±0.19 \\ \midrule
          \multirow{5}{*}{DTD} &      S & \multirow{5}{*}{45.21 ±0.77} &          +0.66 ±0.77 & \multirow{5}{*}{70.10 ±0.59} &          -3.12 ±0.59 & \multirow{5}{*}{76.03 ±0.69} &          -6.67 ±0.69 \\
                               &     TI &                              &          \textbf{+2.85 ±0.46} &                              &          \textbf{+2.77 ±0.33} &                              &          \textbf{+2.44 ±0.29} \\
                               &     DI &                              & \textbf{+2.90 ±0.48} &                              & \textbf{+2.96 ±0.33} &                              &          \textbf{+2.78 ±0.31} \\
                               & DI-UOT &                              &          \textbf{+2.26 ±0.51} &                              &          \textbf{+2.62 ±0.34} &                              & \textbf{+2.82 ±0.32} \\ 
                               
                               & TI-UOT &                               &  \textbf{+2.85 ±0.46} & & \textbf{+2.44 ±0.32} & &  \textbf{+2.82 ±0.32} \\ \midrule
        \multirow{5}{*}{Fungi} &      S & \multirow{5}{*}{53.01 ±0.92} &          -6.59 ±0.74 & \multirow{5}{*}{74.87 ±0.80} &          -8.33 ±0.62 & \multirow{5}{*}{51.57 ±1.16} &         -15.05 ±0.53 \\
                               &     TI &                              &          \textbf{+0.92 ±0.39} &                              &         \textbf{+1.67 ±0.30} &                              &          \textbf{+1.07 ±0.26} \\
                               &     DI &                              & \textbf{+1.07 ±0.41} &                              & \textbf{+1.89 ±0.29} &                              & \textbf{+1.38 ±0.25} \\
                               & DI-UOT &                              &          +0.74 ±0.40 &                              &          \textbf{+1.46 ±0.29} &                              &         \textbf{ +0.91 ±0.25} \\
                               
                               & TI-UOT & & \textbf{+0.92 ±0.39}& &  \textbf{+1.51 ±0.28} & &  +0.80 ±0.25 \\ \midrule
     \multirow{5}{*}{Omniglot} &      S & \multirow{5}{*}{61.80 ±1.03} &          -3.16 ±1.11 & \multirow{5}{*}{81.53 ±0.76} &          \textbf{+3.53 ±0.85} & \multirow{5}{*}{59.51 ±1.31} &          -4.59 ±1.07 \\
                               &     TI &                              &          \textbf{+2.65 ±0.38} &                              &          \textbf{+2.94 ±0.29} &                              &          \textbf{+3.74 ±0.23} \\
                               &     DI &                              & \textbf{+3.52 ±1.22} &                              & \textbf{+3.57 ±0.81} &                              & \textbf{+3.93 ±0.61} \\
                               & DI-UOT &                              &          -3.70 ±1.00 &                              &          -5.02 ±0.68 &                              &          -5.76 ±0.66 \\
                               
                               & TI-UOT & &\textbf{+2.65 ±0.38} & &+2.58 ±0.82& &+2.46 ±0.62\\ \midrule
       \multirow{5}{*}{MSCOCO} &      S & \multirow{5}{*}{43.91 ±0.85} &          -5.44 ±0.66 & \multirow{5}{*}{63.04 ±0.79} &          -6.20 ±0.63 & \multirow{5}{*}{44.99 ±0.99} &         -17.00 ±0.72 \\
                               &     TI &                              &          \textbf{+1.27 ±0.35} &                              &          \textbf{+1.87 ±0.29} &                              &          +1.85 ±0.17 \\
                               &     DI &                              & \textbf{+1.62 ±0.34} &                              & \textbf{+2.09 ±0.30} &                              & \textbf{+2.25 ±0.17} \\
                               & DI-UOT &                              &          \textbf{+1.27 ±0.35} &                              &          \textbf{+1.75 ±0.29} &                              &          \textbf{+2.09 ±0.18} \\
                               
                               & TI-UOT & &\textbf{+1.27 ±0.35} & & +1.30 ±0.28 & & \textbf{+2.05 ±0.18}\\ \midrule
\multirow{5}{*}{Traffic Signs} &      S & \multirow{5}{*}{\textbf{57.35 ±0.85}} &          -4.67 ±0.66 & \multirow{5}{*}{74.11 ±0.78} & \textbf{+6.17 ±0.62} & \multirow{5}{*}{\textbf{53.77 ±1.05}} & \textbf{+0.77 ±1.00} \\
                               &     TI &                              &          \textbf{-0.84 ±0.32} &                              &          -1.22 ±0.25 &                              &          -2.02 ±0.17 \\
                               &     DI &                              &          \textbf{-0.79 ±0.95} &                              &          -1.48 ±0.77 &                              &          -1.82 ±0.44 \\
                               & DI-UOT &                              & \textbf{-0.48 ±0.33} &                              &          -0.64 ±0.27 &                              &          -1.26 ±0.18 \\
                               
                               & TI-UOT & &\textbf{-0.84 ±0.32}& & -0.99 ±0.77& &-1.33 ±0.43 \\ \midrule
   \multirow{5}{*}{VGG Flower} &      S & \multirow{5}{*}{75.86 ±0.84} &          +0.19 ±0.79 & \multirow{5}{*}{94.46 ±0.33} &          -1.45 ±0.37 & \multirow{5}{*}{92.77 ±0.58} &          -5.18 ±0.51 \\
                               &     TI &                              &          \textbf{+2.04 ±0.40} &                              &         \textbf{ +0.64 ±0.18} &                              & \textbf{+1.03 ±0.16} \\
                               &     DI &                              &          \textbf{+1.88 ±0.41} &                              &          \textbf{+0.52 ±0.18} &                              &          \textbf{+0.84 ±0.16} \\
                               & DI-UOT &                              & \textbf{+2.18 ±0.40} &                              & \textbf{+0.67 ±0.18} &                              &          \textbf{+0.90 ±0.16} \\
                               
                               & TI-UOT & & \textbf{+2.04 ±0.40}& &\textbf{+0.90 ±0.17} & &\textbf{+0.95 ±0.16} \\ \midrule
      \multirow{5}{*}{Average} &      S &            \multirow{5}{*}{} &          -5.24 ±0.78 &            \multirow{5}{*}{} &          -3.73 ±0.61 &            \multirow{5}{*}{} &          -7.11 ±0.73 \\
                               &     TI &                              &          \textbf{+1.43 ±0.38} &                              &          \textbf{+1.39 ±0.28} &                              &          \textbf{+1.31 ±0.21} \\
                               &     DI &                              & \textbf{+1.73 ±0.57} &                              & \textbf{+1.55 ±0.41} &                              & \textbf{+1.61 ±0.30} \\
                               & DI-UOT &                              &          +0.63 ±0.47 &                              &          +0.36 ±0.33 &                              &          +0.32 ±0.28 \\
                               & TI-UOT & &	\textbf{+1.43 ±0.36} & & \textbf{+1.10 ±0.44}& & \textbf{+1.21 ±0.32}\\
\bottomrule
\end{tabular}



==> tables/summary_of_methods.tex <==
\begin{tabular}{@{}lcc@{}}
\toprule
\textbf{Information} & \textbf{Data for Finetuning} & \textbf{Feature transform selection} \\
\midrule
\textbf{DI} & \multirow{2}{*}{Source subset selection} &\multirow{3}{*}{N/A} \\
\cmidrule(lr){1-1} 
\multirow{2}{*}{\textbf{TI}} &  &  \\
& Support set & \\
\midrule
\textbf{Agnostic} & Clusters of source classes & Heuristics \\
\bottomrule
\end{tabular}


==> tables/test_results_presentation.tex <==

\begin{tabular}{l l|c|c|c}
\hline
           && 5-ways 1-shot & 5-ways 5-shot & MD \\ \hline
Aircraft
& Baseline   &               &               &    \\
& $\Delta$DI &               &               &    \\
& $\Delta$TI &               &               &    \\
& $\Delta$S &               &               &    \\\hline
CUB
& Baseline   &               &               &    \\
& $\Delta$DI &               &               &    \\
& $\Delta$TI &               &               &    \\
& $\Delta$S &               &               &    \\\hline
& \multicolumn{1}{c|}{\vdots} & \multicolumn{1}{c|}{\vdots} & \multicolumn{1}{c|}{\vdots} & \multicolumn{1}{c}{\vdots} \\ \hline
Average
& Baseline   &               &               &    \\
& $\Delta$DI &               &               &    \\
& $\Delta$TI &               &               &    \\
& $\Delta$S &               &               &    \\\hline
\end{tabular}


